Monaural Audio Speaker Separation with Source Contrastive Estimation

We propose an algorithm to separate simultaneously speaking persons from each other, the "cocktail party problem", using a single microphone. Our approach involves a deep recurrent neural networks regression to a vector space that is descriptive of independent speakers. Such a vector space can embed empirically determined speaker characteristics and is optimized by distinguishing between speaker masks. We call this technique source-contrastive estimation. The methodology is inspired by negative sampling, which has seen success in natural language processing, where an embedding is learned by correlating and de-correlating a given input vector with output weights. Although the matrix determined by the output weights is dependent on a set of known speakers, we only use the input vectors during inference. Doing so will ensure that source separation is explicitly speaker-independent. Our approach is similar to recent deep neural network clustering and permutation-invariant training research; we use weighted spectral features and masks to augment individual speaker frequencies while filtering out other speakers. We avoid, however, the severe computational burden of other approaches with our technique. Furthermore, by training a vector space rather than combinations of different speakers or differences thereof, we avoid the so-called permutation problem during training. Our algorithm offers an intuitive, computationally efficient response to the cocktail party problem, and most importantly boasts better empirical performance than other current techniques.

==> sips-2017/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sips-2017/implementation-archive.tex <==
For this task, all signals were resampled to a rate of $10kHz$. To generate features, all signals scaled to have zero mean and a standard deviation of one.  We apply a preemphasis filter with coefficient $0.095$.   The signals were then converted into short time Fourier transform (STFT) spectrograms. The parameters used were $0.0512 s$ ($512$ sample) Hanning windows of the input waveform with a $0.0256 s$ overlap, computing the discrete Fourier transform (DFT) of the signal in each window, and stacking the resultant spectrograms together to obtain a 2D T-F (Time-Frequency) representation of the signal.  The complex phases $\phi_{t,f}$ were saved separately for use in post separation processing. Separate spectrograms for the signal from each speaker ($s^n_{t,f}$ for $n\in\{1,2,...,M\}$) were computed for training and evaluation purposes, while the total spectrogram was computed by the elementwise sum $s_{t,f}=s^n_{t,f}+s^m_{t,f}$ for two speakers with IDs $n,m$.

The $s_{t,f}$ spectrograms were then passed through a square root nonlinearity and percent normalized.  This is similar to the procedure suggested in \cite{wang2014training}; however we obtained better results with a square root rather than a logarithmic nonlinearity.  This gives the input features for the model as 
\begin{equation}
\label{eqn:input_normalization}
X_{t,f} = \frac{\sqrt{\left|s_{t,f}\right|} - \min{\sqrt{\left|s_{t,f}\right|}}}{\max{\sqrt{\left|s_{t,f}\right|}} - \min{\sqrt{\left|s_{t,f}\right|}}}
\end{equation}

Speaker labels $Y_{t,f}^c$ are assigned to each T-F bin by giving a value of $1$ to the signal which is loudest in at that time and frequency, and a value of $-1$ to all other signals.  
\begin{equation}
Y_{t,f}^c = \left\{
    \begin{aligned}
    &1\text{ if }\text{argmax}(\{\left|s_{t,f}^1\right|,\left|s_{t,f}^\2\right|,...,\left|s_{t,f}^M\right|\})=c \\
    -&1\text{ if }\text{argmax}(\{\left|s_{t,f}^1\right|,\left|s_{t,f}^2\right|,...,\left|s_{t,f}^M\right|\})\neq c
    \end{aligned} \right.
\end{equation}

Batches of size $B=256$ were used in training, which gives input tensors $\mathbf{X}\in\mathbb{R}^{B \times T \times F}$ and label tensors $\mathbf{Y}\in\mathbb{R}^{B \times T \times F \times M}$.  

The algorithm was implemented in Tensorflow. The model consists of two bidirectional long short term memory (BLSTM) layers $r_1, r_2$ of 600 units each followed by a fully connected layer $d_1$ that maps the output of the second BLSTM layer to the input vector space.  The BLSTM layers both use tanh nonlinearities, and the fully connected layer is linear.  For a batch of inputs $\mathbf{X}$, the output of the two BLSTM layers $r_1, r_2 \in \mathbb{R}^{B \times T \times 600}$.  The fully connected linear layer can be implemented as a $1D$ convolution over the $r_2$ output tensor with a filter $w\in\mathbb{R}^{1\times600\times F\cdot E}$.  The output of the convolution can then be reshaped to give the input vector space $\mathbf{V}_i\in\mathbb{R}^{B\times T \times F \times E}$.  This implementation allows the model to be run for arbitrary input $T$, which is useful at inference time.

For efficient evaluation of the cost function of Eq. \ref{eqn:cost} across batches, the speaker vectors for only speakers represented in each batch are assembled into a tensor $\mathbf{V}_o\in\mathbb{R}^{B \times M \times E}$.  Note that for implementation in Tensorflow, version 1.1 or higher is required, because we make extensive use of broadcasting operation (earlier versions of fhe function \verb"gather_nd" do not pass gradients back). The ordering of the $M$ speakers in $\mathbf{V}_o$ must match the ordering used in $\mathbf{Y}$, but is otherwise arbitrary.  To efficiently compute the dot products $V_i\cdot V_o$ in Eq. \ref{eqn:cost},  the dimensions of the input vector space are expanded such that $\mathbf{V}_i\in\mathbb{R}^{B \times T \times F \times 1 \times E}$ and the output vectors have their dimensions expanded so $\mathbf{V}_o\in\mathbb{R}^{B\times 1\times 1 \times M \times E}$.  The dot product can then be computed by doing the elementwise multiplication (broadcasting over the indicies that don't match) and summing over the embedding dimensions.  This gives an output of the dot product operation as a tensor $\mathbf{D}\in\mathbb{R}^{B\times T\times F \times M}$, which is compatable with the labels $\mathbf{Y}$ and so they can be multiplied together elementwise to give the argument of the sigmoid in Eq. \ref{eqn:cost}.  The remaining portion of the cost function is easily evaluated.

At inference time, a signal consisting of an unknown mixture of sources is preprocessed as described above, giving a complex T-F representation of the signal $s_{t,f}$.  An input feature is generated as in Eq. \ref{eqn:input_normalization} and fed through the model to obtain the vectors $\mathbf{V}_i$.  A $K$-means clustering is then performed on the vectors in order to generate a labeling $\mathbf{M}\in\mathbb{R}^{T\times F\times K}$ in which each T-F element is associated with a cluster label.  Here the element $M_{t,f,k}=1$ if the associated vector $V_{t,f}$ belongs to the $k^{th}$ cluster, and $M_{t,f,k}=0$ otherwise.  These labelings can then be used as masks to reconstruct a source $S^k_{t,f}$ from each of the $K$ clusters.  T-F representations of the inferred sources are calculated as the elementwise multiplication of the input spectrogram with the inferred labeling.
\begin{equation}
S^k_{t,f} = s_{t,f}\odot M_{t,f,k}
\end{equation}
The source spectrogram $S^k_{t,f}$ is then converted (using the inverse STFT) into a source waveform and the preemphasis filtering is undone, completing the inference process.

The order of operations is $\mathcal{O}(TFE)$ versus $\mathcal{O}(T^2F^2E)$.

All code involved in our contribution can be found at \verb"http://github.com/lab41/magnolia". 
